Fixed-Capacity Limits of Linearizable Mergeable Cardinality Sketches: Tight Bounds and CapPCSA

Strictly mergeable cardinality sketches evaluate COUNT(DISTINCT) across arbitrary aggregation trees with states bit-identical to sequential union. Variable-length or overflow-prone designs (e.g., Apache CPC and multi-cell Fishmonger) approach Pettie and Wang's linearizable Shannon-entropy floor of 1.980. Yet fixed-width Parquet columns and bounded-slot frames require zero-overflow (delta = 0) fixed wire capacity, where prior fixed-size linearizable sketches suffer memory-variance products (MVPs) strictly above 3.00 on 64-bit universes. We close this gap with three contributions. First, we prove that deterministic fixed capacity raises the asymptotically tight linearizable limits to 2.45926 (+24.2% above 1.980) for inverse-Fisher MVP and 1.82043 (+11.8% above 1.62862) for state-change rate, alongside an implication-DAG criterion and linearizable top-collapse corollary. On matched 64-bit windows, a left-shifted integration window converges at O((ln ln d)/d) and certifies non-vacuous bounds 2.355-2.363. Second, we construct CapPCSA, a pooled-tail PCSA closure matching both limits asymptotically and certifying five 64-bit configurations with inverse-Fisher UB below 3.00 (+14.7%-+25.5% Exact / +14.9%-+26.9% Fast above matched lower bounds), paired with zero-allocation delta = 0 codecs (CapPCSA-Fast, 15.9-34.3 us at g = 2,048 on M5; RawEF). Across 16 real-hash phases, Fast achieves 2.79-2.83 mean MVP (cutting 23.6%-26.5% vs. ExaLogLog-28/32b). Dual-host and Parquet runs map the system trade-offs: CapPCSA leads fixed-wire catalog size and FLBA NONE/LZ4 storage, ties ULL-8b and CPC on 16-phase ZSTD MVP, and trades higher working RAM and small-n hashing cost for provable delta = 0. Third, we prove a continuous smoothed ExaLogLog relaxation diverges as (ln Lambda + ln ln Lambda)/I_0 + O(1) for Lambda = log_2 log_2 U.

==> tables/metrics_macros.tex <==
\makeatletter
\newcommand{\Nm}[1]{\@ifundefined{nm@#1}{\errmessage{Undefined metric macro: #1}}{\csname nm@#1\endcsname}}
\@namedef{nm@asymp.mrg.gap.pct}{0.15}
\@namedef{nm@asymp.mrg.ub}{2.462862}
\@namedef{nm@asymp.rate.gap.pct}{0.17}
\@namedef{nm@asymp.rate.ub}{1.823523}
\@namedef{nm@c.merge.10}{2.4592609211}
\@namedef{nm@c.merge.3}{2.459}
\@namedef{nm@c.merge.5}{2.45926}
\@namedef{nm@c.merge.6}{2.459261}
\@namedef{nm@c.merge.trunc5}{2.45926}
\@namedef{nm@c.merge.trunc6}{2.459260}
\@namedef{nm@c.pw21.3}{1.980}
\@namedef{nm@c.pw21.5}{1.98016}
\@namedef{nm@c.pwy21.5}{1.62862}
\@namedef{nm@c.pwy21.6}{1.628620}
\@namedef{nm@c.rate.10}{1.8204278605}
\@namedef{nm@c.rate.5}{1.82043}
\@namedef{nm@c.rate.6}{1.820428}
\@namedef{nm@c.rate.trunc5}{1.82042}
\@namedef{nm@c.rate.trunc6}{1.820427}
\@namedef{nm@cap.q125.16k.dense}{409{,}144}
\@namedef{nm@cap.q125.16k.ub5}{2.70116}
\@namedef{nm@cap.q125.16k.wire}{37{,}480}
\@namedef{nm@cap.q135.2k.dense}{39{,}072}
\@namedef{nm@cap.q135.2k.ram}{6{,}602}
\@namedef{nm@cap.q135.2k.ramcut}{5.92}
\@namedef{nm@cap.q135.2k.ub2}{2.90}
\@namedef{nm@cap.q135.2k.ub5}{2.89749}
\@namedef{nm@cap.q135.2k.wire}{3{,}757}
\@namedef{nm@cap.q15.2k.ub5}{2.96512}
\@namedef{nm@cap.q15.2k.wire}{2{,}812}
\@namedef{nm@cat.curt.mb}{342.4}
\@namedef{nm@cat.ell32.mb}{409.6}
\@namedef{nm@cat.fast135.mb}{379.3}
\@namedef{nm@cat.fast15.cut.curt.pct}{17.0}
\@namedef{nm@cat.fast15.cut.ell.pct}{30.6}
\@namedef{nm@cat.fast15.mb}{284.3}
\@namedef{nm@cat.r16.cpc12}{593.1}
\@namedef{nm@cat.r16.curt}{728.8}
\@namedef{nm@cat.r16.ell32}{76.8}
\@namedef{nm@cat.r16.exact.ms}{105.4}
\@namedef{nm@cat.r16.exact.speedup}{183}
\@namedef{nm@cat.r16.fast15}{574.6}
\@namedef{nm@cat.r16.fast15.vs.cpc}{1.03}
\@namedef{nm@cat.r16.fast15.vs.ullz}{0.70}
\@namedef{nm@cat.r16.rawef}{235.8}
\@namedef{nm@cat.r16.rawef.vs.curt}{3.09}
\@namedef{nm@cat.r16.rawef15}{146.4}
\@namedef{nm@cat.r16.ull}{48.4}
\@namedef{nm@cat.r16.ullz}{405.0}
\@namedef{nm@cat.r256.cpc12}{11.09}
\@namedef{nm@cat.r256.curt}{9.08}
\@namedef{nm@cat.r256.exact.ms}{1756.6}
\@namedef{nm@cat.r256.exact.speedup}{128}
\@namedef{nm@cat.r256.fast15}{13.71}
\@namedef{nm@cat.r256.fast15.dec.ms}{12.62}
\@namedef{nm@cat.r256.fast15.dec.pct}{92.0}
\@namedef{nm@cat.r256.rawef}{5.06}
\@namedef{nm@cat.r256.rawef15}{3.18}
\@namedef{nm@cat.r256.ull}{324.2}
\@namedef{nm@cat.r256.ullz}{8.31}
\@namedef{nm@cat.r64.cpc12}{2{,}262.4}
\@namedef{nm@cat.r64.curt}{2{,}646.5}
\@namedef{nm@cat.r64.fast15}{3{,}160.3}
\@namedef{nm@cat.r64.rawef}{1{,}201.8}
\@namedef{nm@cat.r64.rawef15}{611.2}
\@namedef{nm@cat.r64.ullz}{1{,}580.1}
\@namedef{nm@cat.rawef.vs.cpc.max}{2.5}
\@namedef{nm@cat.rawef.vs.cpc.min}{1.9}
\@namedef{nm@cat.rawef.vs.ullz.max}{1.7}
\@namedef{nm@cat.rawef.vs.ullz.min}{1.3}
\@namedef{nm@cat.rawef135.mb}{399.0}
\@namedef{nm@cat.rawef15.mb}{298.9}
\@namedef{nm@cat.rawef15.vs.cpc.max}{4.1}
\@namedef{nm@cat.rawef15.vs.cpc.min}{3.5}
\@namedef{nm@cat.rawef15.vs.ullz.max}{2.8}
\@namedef{nm@cat.rawef15.vs.ullz.min}{2.6}
\@namedef{nm@cpc11.ins.ns}{36.5}
\@namedef{nm@cpc12.16k.maxb}{2{,}568}
\@namedef{nm@cpc12.dec.us}{23.2}
\@namedef{nm@cpc12.empcap.b}{2{,}580}
\@namedef{nm@cpc12.ins.ns}{52.4}
\@namedef{nm@cpc12.live}{5{,}120}
\@namedef{nm@cpc12.mean.b}{2488.6}
\@namedef{nm@cpc12.mrg.peak}{65{,}536}
\@namedef{nm@cpc12.mrg.us}{21.3}
\@namedef{nm@cpc12.mvp}{2.3669}
\@namedef{nm@cpc12.p99}{2.73}
\@namedef{nm@cpc12.peak}{37{,}888}
\@namedef{nm@cpc12.peak.ratio}{5.74}
\@namedef{nm@cpc12.sp16k.mean.b}{2492.8}
\@namedef{nm@cpc12.sp16k.ph.hi}{2496.1}
\@namedef{nm@cpc12.sp16k.ph.lo}{2488.8}
\@namedef{nm@cpc12.sp2500.delta}{33.3}
\@namedef{nm@cpc12.sp2500.mvp}{3.12}
\@namedef{nm@cpc12.sp2560.ov}{10}
\@namedef{nm@cpc12.sp2580.mvp}{2.41}
\@namedef{nm@cpc12.uncomp.b}{32{,}768}
\@namedef{nm@cpc13.ins.ns}{43.5}
\@namedef{nm@curtain.3b.mvp}{3.26}
\@namedef{nm@curtain.int.mvp}{3.15}
\@namedef{nm@cut.fast.2k.curt.pct}{14.5}
\@namedef{nm@cut.fast.2k.ell32.pct}{28.0}
\@namedef{nm@cut.fast.4k.curt.pct}{18.9}
\@namedef{nm@cut.fast.4k.ell32.pct}{27.3}
\@namedef{nm@d1e6.mrg.elem.5}{2.45925}
\@namedef{nm@d64.cI.arb.5}{2.44930}
\@namedef{nm@d64.cR.arb.5}{1.81349}
\@namedef{nm@d64.mrg.arb.3}{2.382}
\@namedef{nm@d64.mrg.arb.6}{2.382768}
\@namedef{nm@d64.mrg.arb.int.3}{2.380}
\@namedef{nm@d64.mrg.arb.pct}{20.3}
\@namedef{nm@d64.mrg.elem.3}{2.355}
\@namedef{nm@d64.mrg.elem.int.3}{2.351}
\@namedef{nm@d64.mrg.elem.int175.3}{2.351}
\@namedef{nm@d64.mrg.elem.pct}{19.0}
\@namedef{nm@d64.rate.arb.3}{1.778}
\@namedef{nm@d64.rate.arb.6}{1.778321}
\@namedef{nm@d64.rate.arb.int.3}{1.777}
\@namedef{nm@d64.rate.arb.pct}{9.2}
\@namedef{nm@d64.rate.elem.3}{1.757}
\@namedef{nm@d64.rate.elem.pct}{7.9}
\@namedef{nm@d64.val}{42.98}
\@namedef{nm@ell.fstar.1e300}{7.09}
\@namedef{nm@ell.fstar.64}{3.6716}
\@namedef{nm@ell.fstar.64.2}{3.67}
\@namedef{nm@ell.res2.1e300}{1.718}
\@namedef{nm@ell.res2.1e300.lo}{1.717}
\@namedef{nm@ell.res2.32}{2.262}
\@namedef{nm@ell.res2.32.hi}{2.262}
\@namedef{nm@ell.res2.64}{2.228}
\@namedef{nm@ell.twoterm.64}{1.444}
\@namedef{nm@elleq.ci.hi}{0.618}
\@namedef{nm@elleq.ci.lo}{-0.869}
\@namedef{nm@elleq.max.z}{1.70}
\@namedef{nm@elleq.pair.hi}{0.565}
\@namedef{nm@elleq.pair.lo}{-0.688}
\@namedef{nm@elleq.pair.max.z}{1.70}
\@namedef{nm@fast.fig1.ovh.max}{1.10}
\@namedef{nm@fast.fig1.ovh.min}{0.60}
\@namedef{nm@fast.lut.orbit.layer}{84}
\@namedef{nm@fast.lut.orbit.max.kb}{2.18}
\@namedef{nm@fast.lut.orbit.min.kb}{0.59}
\@namedef{nm@fast.lut.rans.max.kb}{9.8}
\@namedef{nm@fast.lut.rans.min.kb}{2.6}
\@namedef{nm@fast.ovh.max}{1.47}
\@namedef{nm@fast.ovh.min}{0.23}
\@namedef{nm@fast.q125.16k.ovh}{0.23}
\@namedef{nm@fast.q125.16k.ub5}{2.70750}
\@namedef{nm@fast.q135.2k.ub2}{2.93}
\@namedef{nm@fast.q135.2k.ub5}{2.92525}
\@namedef{nm@fast.q135.2k.wire}{3{,}793}
\@namedef{nm@fast.q15.2k.ovh}{1.10}
\@namedef{nm@fast.q15.2k.ub3}{2.998}
\@namedef{nm@fast.q15.2k.ub5}{2.99781}
\@namedef{nm@fast.q15.2k.wire}{2{,}843}
\@namedef{nm@fast.spd.2k.max}{333}
\@namedef{nm@fast.spd.2k.min}{237}
\@namedef{nm@fast.spd.max}{1{,}865}
\@namedef{nm@fast.spd.min}{218}
\@namedef{nm@fast.static.max.kb}{16.1}
\@namedef{nm@fast.static.min.kb}{4.7}
\@namedef{nm@h0.6}{3.257240}
\@namedef{nm@hupper.6}{2.088566}
\@namedef{nm@i0.6}{1.644934}
\@namedef{nm@lat.id157.pen}{2.1}
\@namedef{nm@lat.id159.ub}{2.3324}
\@namedef{nm@lat.id165.pen}{2.7}
\@namedef{nm@lat.id166.ub}{3.0629}
\@namedef{nm@lat.id212.pen}{159.6}
\@namedef{nm@lat.id218.pen}{6.2}
\@namedef{nm@lat.lin}{38}
\@namedef{nm@lat.nonlin}{261}
\@namedef{nm@lat.total}{299}
\@namedef{nm@mle.speedup.2k}{8.5}
\@namedef{nm@mw.gap.q2.ex}{34.5}
\@namedef{nm@mw.gap.q2.fa}{36.5}
\@namedef{nm@mw.gap5.ex.hi}{25.5}
\@namedef{nm@mw.gap5.ex.lo}{14.7}
\@namedef{nm@mw.gap5.fa.hi}{26.9}
\@namedef{nm@mw.gap5.fa.lo}{14.9}
\@namedef{nm@mw.hi.3}{2.363}
\@namedef{nm@mw.lo.3}{2.355}
\@namedef{nm@mw.pct.hi}{19.4}
\@namedef{nm@mw.pct.lo}{19.0}
\@namedef{nm@mw.q135.2k.3}{2.362}
\@namedef{nm@mw.q15.2k.3}{2.362}
\@namedef{nm@olap.cut.15.ell32}{30.6}
\@namedef{nm@olap.dense.bw.e2e.ell32}{2.0}
\@namedef{nm@olap.dense.bw.e2e.ull}{2.0}
\@namedef{nm@olap.dense.bw.ell32}{59}
\@namedef{nm@olap.dense.bw.ull}{58}
\@namedef{nm@olap.dense.ell32.mb}{8.39}
\@namedef{nm@olap.dense.exact15.s}{26.65}
\@namedef{nm@olap.dense.fast15.mb}{5.82}
\@namedef{nm@olap.dense.fast15.ms}{358.5}
\@namedef{nm@olap.dense.rawef.ms}{88.7}
\@namedef{nm@olap.dense.rawef.speedup}{300}
\@namedef{nm@olap.dense.rawef15.bw.ell32}{337}
\@namedef{nm@olap.dense.rawef15.bw.ull}{294}
\@namedef{nm@olap.dense.rawef15.ms}{64.8}
\@namedef{nm@olap.dense.speedup}{74}
\@namedef{nm@olap.dense.ullz.ms}{188.2}
\@namedef{nm@olap.ell32.mb}{134.22}
\@namedef{nm@olap.events}{14{,}080{,}000}
\@namedef{nm@olap.fast135.mb}{124.29}
\@namedef{nm@olap.fast15.mb}{93.16}
\@namedef{nm@olap.sketches}{32{,}768}
\@namedef{nm@olap.sparse.cpc12.cm}{0.591}
\@namedef{nm@olap.sparse.cpc12.mb}{9.38}
\@namedef{nm@olap.sparse.cpc12.rmse}{0.69}
\@namedef{nm@olap.sparse.ell32.e2e}{2.022}
\@namedef{nm@olap.sparse.ell32.rmse}{0.795}
\@namedef{nm@olap.sparse.fast15.e2e}{4.466}
\@namedef{nm@olap.sparse.fast15.rmse}{0.775}
\@namedef{nm@olap.sparse.rawef.e2e}{3.779}
\@namedef{nm@olap.sparse.rawef.rmse.all}{0.649}
\@namedef{nm@olap.sparse.rawef.rmse.hvy}{0.713}
\@namedef{nm@olap.sparse.ull.e2e}{1.800}
\@namedef{nm@olap.sparse.ull.rmse}{0.874}
\@namedef{nm@olap.sparse.ullz.mb}{15.33}
\@namedef{nm@ops.cap.exact.max}{33{,}406}
\@namedef{nm@ops.cap.exact.min}{4{,}084}
\@namedef{nm@ops.cap.mrg.max}{4.00}
\@namedef{nm@ops.cap.mrg.min}{2.46}
\@namedef{nm@ops.cap.vs.cpc.dec}{0.71}
\@namedef{nm@ops.cap.vs.cpc.ins}{5.9}
\@namedef{nm@ops.cap.vs.cpc.mrg.max}{8.7}
\@namedef{nm@ops.cap.vs.cpc.mrg.min}{5.3}
\@namedef{nm@ops.cap.vs.curt.max}{12.5}
\@namedef{nm@ops.cap.vs.curt.min}{7.7}
\@namedef{nm@ops.cap.vs.ull.max}{0.5}
\@namedef{nm@ops.cap.vs.ull.min}{0.3}
\@namedef{nm@ops.cap135.2k.ef.dec}{10.5}
\@namedef{nm@ops.cap135.2k.ef.enc}{9.5}
\@namedef{nm@ops.cap135.2k.fast.dec}{34.3}
\@namedef{nm@ops.cap135.2k.fast.enc}{22.5}
\@namedef{nm@ops.cap135.2k.ins}{12.33}
\@namedef{nm@ops.cap135.2k.mle}{3.20}
\@namedef{nm@ops.cap135.2k.mrg}{3.29}
\@namedef{nm@ops.cap135.4k.mrg}{4.00}
\@namedef{nm@ops.cap15.2k.ef.dec}{6.3}
\@namedef{nm@ops.cap15.2k.ef.enc}{5.7}
\@namedef{nm@ops.cap15.2k.fast.dec}{32.5}
\@namedef{nm@ops.cap15.2k.fast.dec.iqr}{24.7--32.9}
\@namedef{nm@ops.cap15.2k.fast.enc}{15.9}
\@namedef{nm@ops.cap15.2k.fast.enc.iqr}{15.8--16.1}
\@namedef{nm@ops.cap15.2k.ins}{8.90}
\@namedef{nm@ops.cap15.2k.mle}{2.39}
\@namedef{nm@ops.cap15.2k.mrg}{3.12}
\@namedef{nm@ops.cap15.2k.mrg.iqr}{3.12--3.12}
\@namedef{nm@ops.curt4k.dec}{18.8}
\@namedef{nm@ops.curt4k.enc}{32.7}
\@namedef{nm@ops.curt4k.mrg}{30.6}
\@namedef{nm@ops.ef.vs.cpc.dec}{2.2}
\@namedef{nm@ops.ell32.1k.ins}{10.00}
\@namedef{nm@ops.ell32.1k.mle}{27.3}
\@namedef{nm@ops.ell32.1k.mrg}{3.17}
\@namedef{nm@ops.reg.ins.max}{10.0}
\@namedef{nm@ops.reg.ins.min}{4.0}
\@namedef{nm@ops.ull4k.mrg}{1.25}
\@namedef{nm@ops.zstd.ell.enc}{58.2}
\@namedef{nm@ops.zstd.ull.dec}{16.4}
\@namedef{nm@ops.zstd.ull.enc}{48.5}
\@namedef{nm@p16.q135.2k.fast.ci}{2.9268}
\@namedef{nm@p16.q135.2k.fast.max}{2.8650}
\@namedef{nm@p16.q135.4k.fast.ci}{2.8533}
\@namedef{nm@p16.q135.4k.fast.max}{2.7920}
\@namedef{nm@p16.q15.2k.fast.ci}{2.9890}
\@namedef{nm@p16.q15.2k.fast.max}{2.9256}
\@namedef{nm@p16.q15.4k.fast.ci}{2.8840}
\@namedef{nm@p16.q15.4k.fast.max}{2.8219}
\@namedef{nm@p16.realhash.ex.max}{2.8770}
\@namedef{nm@p16.realhash.fast.max}{2.9046}
\@namedef{nm@pair.fast2k.curt.z}{-6.28}
\@namedef{nm@pair.fast2k.ell32.z}{-11.91}
\@namedef{nm@pair.fast4k.curt.z}{-8.18}
\@namedef{nm@pair.fast4k.ell32.z}{-12.04}
\@namedef{nm@pct.above.pw21.1}{24.2}
\@namedef{nm@pct.above.pw21.3}{24.195}
\@namedef{nm@pct.above.pwy21.1}{11.8}
\@namedef{nm@pct.above.pwy21.3}{11.777}
\@namedef{nm@ph.b16.curt.max}{3.425}
\@namedef{nm@ph.b16.curt.mean}{3.277}
\@namedef{nm@ph.b16.curt.mean2}{3.28}
\@namedef{nm@ph.b16.ell28.mean}{3.703}
\@namedef{nm@ph.b16.ell28.mean2}{3.70}
\@namedef{nm@ph.b16.ell32.max}{3.944}
\@namedef{nm@ph.b16.ell32.mean}{3.788}
\@namedef{nm@ph.b16.ell32.mean2}{3.79}
\@namedef{nm@ph.b16.fast135.ci2}{3.10}
\@namedef{nm@ph.b16.fast135.max}{2.913}
\@namedef{nm@ph.b16.fast135.mean}{2.785}
\@namedef{nm@ph.b16.fast135.mean2}{2.79}
\@namedef{nm@ph.b16.fast15.ci2}{3.18}
\@namedef{nm@ph.b16.fast15.max}{2.994}
\@namedef{nm@ph.b16.fast15.mean}{2.829}
\@namedef{nm@ph.b16.fast15.mean2}{2.83}
\@namedef{nm@ph.b16.ull.max}{4.793}
\@namedef{nm@ph.b16.ull.mean}{4.567}
\@namedef{nm@ph.cut.fast135.curt}{15.0}
\@namedef{nm@ph.cut.fast135.ell28}{24.8}
\@namedef{nm@ph.cut.fast135.ell32}{26.5}
\@namedef{nm@ph.cut.fast15.curt}{13.7}
\@namedef{nm@ph.cut.fast15.ell28}{23.6}
\@namedef{nm@ph.cut.fast15.ell32}{25.3}
\@namedef{nm@pq.s.cpc.zstd}{1425.8}
\@namedef{nm@pq.s.rawef15.lz4}{1683.3}
\@namedef{nm@pq.s.rawef15.zstd}{1473.4}
\@namedef{nm@pq.s.ull.lz4}{2522.0}
\@namedef{nm@pq.s.ull.zstd}{1570.9}
\@namedef{nm@pq.u.cpc.zstd}{2493.4}
\@namedef{nm@pq.u.cpc.zstd.mvp16}{2.33}
\@namedef{nm@pq.u.curt.zstd.mvp16}{3.01}
\@namedef{nm@pq.u.ell32.zstd.mvp16}{2.91}
\@namedef{nm@pq.u.fast135.zstd.mvp16}{2.26}
\@namedef{nm@pq.u.fast15.lz4}{2407.2}
\@namedef{nm@pq.u.fast15.none}{2843.0}
\@namedef{nm@pq.u.fast15.zstd}{2291.7}
\@namedef{nm@pq.u.fast15.zstd.mvp16}{2.28}
\@namedef{nm@pq.u.rawef15.zstd}{2453.7}
\@namedef{nm@pq.u.rawef15.zstd.mvp16}{2.44}
\@namedef{nm@pq.u.ull.lz4}{4021.4}
\@namedef{nm@pq.u.ull.zstd}{2066.2}
\@namedef{nm@pq.u.ull.zstd.mvp16}{2.30}
\@namedef{nm@pq.u.ullz.zstd.mvp16}{2.46}
\@namedef{nm@race.q125.16k.fast.dec}{438.9}
\@namedef{nm@race.q125.16k.fast.enc}{298.0}
\@namedef{nm@race.q135.2k.bw.fast}{42}
\@namedef{nm@race.q135.2k.ef.dec}{10.9}
\@namedef{nm@race.q135.2k.exact.dec.ms}{8.6}
\@namedef{nm@race.q135.2k.fast.dec}{36.1}
\@namedef{nm@race.q135.2k.fast.enc}{22.3}
\@namedef{nm@race.q15.2k.bw.32c.gbps}{4.8}
\@namedef{nm@race.q15.2k.bw.fast}{151}
\@namedef{nm@race.q15.2k.ef.enc}{6.2}
\@namedef{nm@race.q15.2k.exact.enc.ms}{5.3}
\@namedef{nm@race.q15.2k.fast.dec}{25.0}
\@namedef{nm@race.q15.2k.fast.enc}{15.9}
\@namedef{nm@ramcut.max}{6.21}
\@namedef{nm@ramcut.min}{5.65}
\@namedef{nm@ramcut.sub3.max}{6.07}
\@namedef{nm@ramcut.sub3.min}{5.65}
\@namedef{nm@rawef.q125.16k.ub3}{2.859}
\@namedef{nm@rawef.q135.2k.ub3}{3.078}
\@namedef{nm@rawef.q135.2k.wire}{3{,}990}
\@namedef{nm@rawef.q135.4k.ub3}{2.999}
\@namedef{nm@rawef.q135.4k.ub5}{2.99826}
\@namedef{nm@rawef.q15.2k.ub3}{3.152}
\@namedef{nm@rawef.q15.4k.ub3}{3.073}
\@namedef{nm@reg.dup8.ell32}{12.7}
\@namedef{nm@reg.dup8.fast15}{17.1}
\@namedef{nm@reg.n100.fast15}{39.2}
\@namedef{nm@reg.n10k.fast15}{44.8}
\@namedef{nm@reg.n1m.ell32}{8.66}
\@namedef{nm@reg.n1m.fast15}{9.91}
\@namedef{nm@reg.pre.ell32}{6.6}
\@namedef{nm@reg.pre.fast15}{29.2}
\@namedef{nm@reg.ratio.dup8}{1.34}
\@namedef{nm@reg.ratio.n100}{5.53}
\@namedef{nm@reg.ratio.n10k}{4.45}
\@namedef{nm@reg.ratio.n1m}{1.14}
\@namedef{nm@reg.ratio.pre}{4.40}
\@namedef{nm@reg.x86.ratio.max}{5.31}
\@namedef{nm@reg.x86.ratio.min}{1.08}
\@namedef{nm@root.spur.merge}{0.250}
\@namedef{nm@root.spur.rate}{0.271}
\@namedef{nm@s1m.cap135.2k.mvp}{2.6967}
\@namedef{nm@s1m.cap135.2k.mvp2}{2.70}
\@namedef{nm@s1m.cap135.4k.mvp}{2.6100}
\@namedef{nm@s1m.cap135.4k.mvp2}{2.61}
\@namedef{nm@s1m.cap15.2k.mvp2}{2.63}
\@namedef{nm@s1m.curt4k.mvp}{3.1825}
\@namedef{nm@s1m.curt4k.mvp2}{3.18}
\@namedef{nm@s1m.curt8k.mvp}{3.2392}
\@namedef{nm@s1m.curt8k.mvp2}{3.24}
\@namedef{nm@s1m.cut.t2.ell28}{26.2}
\@namedef{nm@s1m.ell28.1k.mvp}{3.7247}
\@namedef{nm@s1m.ell28.2k.mvp}{3.5561}
\@namedef{nm@s1m.ell28.2k.mvp2}{3.56}
\@namedef{nm@s1m.ell32.1k.mvp}{3.7815}
\@namedef{nm@s1m.ell32.1k.mvp2}{3.78}
\@namedef{nm@s1m.ell32.2k.mvp}{3.6122}
\@namedef{nm@s1m.ell32.ram.mvp.hi}{3.78}
\@namedef{nm@s1m.ell32.ram.mvp.lo}{3.61}
\@namedef{nm@s1m.fast.ram.mvp.hi}{4.74}
\@namedef{nm@s1m.fast.ram.mvp.lo}{4.47}
\@namedef{nm@s1m.fast135.2k.mvp}{2.7226}
\@namedef{nm@s1m.fast135.2k.mvp2}{2.72}
\@namedef{nm@s1m.fast135.2k.rmse2}{0.95}
\@namedef{nm@s1m.fast135.2k.rmse3}{0.947}
\@namedef{nm@s1m.fast135.2k.se}{0.0598}
\@namedef{nm@s1m.fast135.4k.mvp}{2.6256}
\@namedef{nm@s1m.fast135.4k.mvp2}{2.63}
\@namedef{nm@s1m.fast15.2k.cut4k.pct}{30.6}
\@namedef{nm@s1m.fast15.2k.mvp2}{2.65}
\@namedef{nm@s1m.fast15.4k.mvp2}{2.76}
\@namedef{nm@s1m.hll.4k.mvp2}{6.39}
\@namedef{nm@s1m.rawef135.2k.mvp3}{2.864}
\@namedef{nm@s1m.rawef135.4k.mvp3}{2.764}
\@namedef{nm@s1m.rawef15.2k.mvp3}{2.790}
\@namedef{nm@s1m.ull.4k.fb.mvp3}{4.596}
\@namedef{nm@s1m.ull.4k.mvp}{4.5948}
\@namedef{nm@s1m.ull.8k.mvp}{4.5150}
\@namedef{nm@s1m.zstd.ell32.1k.bytes}{3272.5}
\@namedef{nm@s1m.zstd.ell32.1k.mvp}{3.0212}
\@namedef{nm@s1m.zstd.ell32.1k.mvp2}{3.02}
\@namedef{nm@s1m.zstd.ull4k.bytes}{2235.0}
\@namedef{nm@s1m.zstd.ull4k.mvp}{2.5072}
\@namedef{nm@small.cells}{52}
\@namedef{nm@small.dcap.hi}{0.0009}
\@namedef{nm@small.dcap.lo}{0.0008}
\@namedef{nm@small.lmin.p.hi}{0.0010}
\@namedef{nm@small.lmin.p.lo}{0.0003}
\@namedef{nm@small.max.bias}{0.022}
\@namedef{nm@small.max.mvp}{1.81}
\@namedef{nm@small.pos.cells}{36}
\@namedef{nm@small.trials}{208{,}000}
\@namedef{nm@st.b6.slot.hi}{3.03}
\@namedef{nm@st.b6.slot.lo}{3.02}
\@namedef{nm@st.b6.worst.hi}{3.12}
\@namedef{nm@t.merge.4}{3.3579}
\@namedef{nm@t.merge.6}{3.357948}
\@namedef{nm@t.rate.4}{1.9705}
\@namedef{nm@t.rate.6}{1.970512}
\@namedef{nm@t.turn.i}{1.5936}
\@namedef{nm@thm3.trans}{14{,}745{,}600}
\@namedef{nm@tree.cpc.n}{1{,}200}
\@namedef{nm@tree.rust.n}{4{,}000}
\@namedef{nm@ullz.16k.maxb}{2{,}268}
\@namedef{nm@ullz.16ph.mvp}{2.46}
\@namedef{nm@ullz.sp2400.mvp}{2.64}
\@namedef{nm@xeon.cap135.mrg}{3.60}
\@namedef{nm@xeon.cap15.ef.dec}{7.5}
\@namedef{nm@xeon.cap15.ef.enc}{6.2}
\@namedef{nm@xeon.cap15.fast.dec}{32.0}
\@namedef{nm@xeon.cap15.fast.enc}{19.3}
\@namedef{nm@xeon.cap15.ins}{8.49}
\@namedef{nm@xeon.cap15.mrg}{2.49}
\@namedef{nm@xeon.cpc.ins.ratio}{2.3}
\@namedef{nm@xeon.cpc12.mrg}{31.4}
\@namedef{nm@xeon.curt4k.mrg}{26.7}
\@namedef{nm@xeon.dense.cpc12.ms}{158.0}
\@namedef{nm@xeon.dense.rawef15.ms}{61.4}
\@namedef{nm@xeon.ell32.mrg}{0.75}
\@namedef{nm@xeon.hll4k.mrg}{0.11}
\@namedef{nm@xeon.mrg.q135.ell}{4.8}
\@namedef{nm@xeon.mrg.q135.hll}{31.6}
\@namedef{nm@xeon.mrg.q15.max}{21.8}
\@namedef{nm@xeon.mrg.q15.min}{3.3}
\@namedef{nm@xeon.r16.rawef15}{191.1}
\@namedef{nm@xeon.r256.cpc12.ms}{9.05}
\@namedef{nm@xeon.r256.rawef15.ms}{3.26}
\@namedef{nm@xeon.r256.ullz.ms}{2.75}
\@namedef{nm@xeon.spd.max}{378}
\@namedef{nm@xeon.spd.min}{60}
\@namedef{nm@xeon.ull4k.mrg}{0.54}
\makeatother

